A stable path to ferromagnetic hydrogenated graphene growth

In this paper, we propose a practical way to stabilize half-hydrogenated graphene (graphone). We show that the dipole moments induced by an hexagonal-boron nitride (h-BN) substrate on graphene stabilize the hydrogen atoms on one sublattice of the graphene layer and suppress the migration of the absorbed hydrogen atoms. Based upon first principle spin polarized density of states (DOS) calculations, we show that the half hydrogenated graphene (graphone) obtained in different graphene-h-BN heterostructures exhibits a half metallic state. We propose to use this new exotic material for spin valve and other spintronics devices and applications.

==> Abstract.tex <==
\begin{abstract}
In this paper we propose a practical way to fabricate 
half-hydrogenated graphene (graphone). 
We show that the dipole moments induced by graphene on hexagonal-boron 
nitride (h-BN) substrate  stabilize the hydrogen atoms on one sublattice 
of the graphene layer and  enhance the  migration barrier for 
the absorbed hydrogen atoms. Using first principle spin polarized density of 
states (DOS) calculations, we show  that the half hydrogenated 
graphene (graphone) obtained in different graphene-h-Bn heterostructures  
exhibits a half metallic state. We propose to use this new exotic material
for  spin valve devices and other spintronic applications.
\end{abstract}

